How the Experts Do It: Assessing and Explaining Agent Behaviors in Real-Time Strategy Games

How should an AI-based explanation system explain an agent's complex behavior to ordinary end users who have no background in AI? Answering this question is an active research area, for if an AI-based explanation system could effectively explain intelligent agents' behavior, it could enable the end users to understand, assess, and appropriately trust (or distrust) the agents attempting to help them. To provide insights into this question, we turned to human expert explainers in the real-time strategy domain, "shoutcaster", to understand (1) how they foraged in an evolving strategy game in real time, (2) how they assessed the players' behaviors, and (3) how they constructed pertinent and timely explanations out of their insights and delivered them to their audience. The results provided insights into shoutcasters' foraging strategies for gleaning information necessary to assess and explain the players; a characterization of the types of implicit questions shoutcasters answered; and implications for creating explanations by using the patterns

==> leftovers.tex <==
\section{LEFTOVERS, DO NOT BE RENDERING THIS SECTION IN FINAL COPY}

Content code analysis showed that content subcodes varied in frequency and consistency between \Spair{Pairs}.
The most frequently described \Ccode{objects} were \Ccode{fighting object}, \Ccode{production object}, and \Ccode{enemy}, while the most frequently described \Ccode{actions} were \Ccode{fighting} and \Ccode{building/producing.}
In order to know how the explanation system should structure sentences, co-occurrence results show us which verbs, nouns, and adjectives/adverbs appear together.


Within \Ccode{object} codes, specified numbers tend to be used when describing objects of higher value to the player and unspecified numbers tend to be used when describing objects of lower value. 
These results can be used when guiding the development of a future explanation system, by demonstrating what vocabulary to use and how to structure the sentences. 
While it is more informative for \Spair{Pairs} to enumerate the unit types and quantities, \Spair{Pairs} have to provide their commentary in real time and cannot always discover or provide these details. 

**this is a leftover from the Intro:

In this work, we studied how commentators exposed depth as applied to \emph{human} agent actions to understand how we should expose depth of \emph{intelligent} agent actions.
This choice was made because from the shoutcaster's perspective, human and intelligent agent actions are almost indistinguishable since they only get to observe the environment anyway.
Further, generating explanations of intelligent agent actions remains an open research area.
This means that there is a paucity of explanations of that type to analyze, particularly in that shoutcaster commentary for intelligent agents playing Starcraft is not available.

---

%\boldify{Another case of high specificity: spellcasters counts are ID. Perhaps because they are DERIVABLE, due to being singular or otherwise small in number. }

%However, there were times when specific numbers were provided when they were not accessible, namely when the number was easy to \emph{derive}.
%``Spellcaster'' units illustrate this well because they are usually present in small numbers; the largest number of precisely specified spellcaster units in the corpus was three.
%The set of observed spellcaster units \{oracle, infestor, mothership core, phoenix, sentry, raven, overseer, ravager\} was quantified discretely 18 times in the corpus, only 4 of which were \Ccode{unidentified discrete}.
%This indicates that when the number is small, the \Spair{Pair} may be willing to count if the information is not accessible.
%To further corroborate this, consider that when cheap military units are precisely quantified, they are often small numbers; 9 of the 20 \Ccode{identified discrete} quantifications of such units were two or less.
%\FIXME{Does this paragraph need a quote? doesnt really feel like it fits but there isnt one in it.}


\boldify{PRELIMINARY: Ordering seems like it should also illuminate things, but we need to do more digging to deliver on this boldify (probably do not have time)}

There were a few options in the ``Tab'' (region 3 of Figure~\ref{fig:gameScreenshot}), which offered details on demand to support drilling down, along with the passively available patches.

What was the difference between the rarely-used past performance measures and the more often-used present performance measures?
All of the past performance measures were ``high aggregation'', such as the sum of resource value of units that have died, shown on the Units Lost tab in Figure~\ref{fig:performance}.
In contrast, Table 2** also shows that the performance measures that were heavily used were all ``low'' aggregation patches, such as 

\boldify{Repetition and action building/producing have high co-occurrence. There are a variety of explanations that contribute to this, such as making an additional base, producing more unspecified units, and remaking something.}

\Ccode{Repetition} and \Ccode{action building/producing} had a high co-occurrence of 18\% and there were 68 instances of this co-occurrence.
There were a variety of explanations that contributed to co-occurrences of these two codes.
One type of explanation was referring to players making their $n^{th}$ base, such as: \quotate{5}{He's making a 5th base now...}
Shoutcasters also referred to players building several units, without specifying the exact unit type.
An example of this was: \quotate{4}{...so we do see DeMusliM just cranking out units.}
Another type of explanation that involved both \Ccode{repetition} and \Ccode{action building/producing} was remaking something, such as \quotate{4}{...now having to remake that entire upgrade}

In our corpus there were 24 instances of co-occurrences of \Ccode{spatial arrangement} and \Ccode{production object} subcodes.
Of these 24 instances 6 were related to pylons, which are objects that provide players with addtional capacity to build units.
One example is \quotate{1}{...the one place you don't have a pylon is where terran is going to setup as soon as they drop your base}

To inform an explanation system of when it needs to specify individual units numbers, we looked through \Spair{Pair} utterances to distinguish objects that are described using unspecified numbers, as opposed to specific numbers.

%\boldify{We should distinguish objects that are described using unspecified numbers, as opposed to specific numbers.  This will allow us to inform the explanation system of when it needs to specifiy individual unit numbers. We found that high value objects such as workers are described precisely, while units of lower value such as marines are described inprecisely. This makes sense, because in a unit has low value you don't care about the exact number.}

Figure~\ref{table:coOccurrence} shows that co-occurrence rates across the \Ccode{identified discrete} and \Ccode{unidentified discrete} columns were similar, with the exception of \Ccode{production object}, \Ccode{upgrade object}, and \Ccode{action building/producing}.
The co-occurrence rate for \Ccode{quantity identified discrete} and \Ccode{action building/producing} was 20\%, which was much higher than the rate of 7\% for \Ccode{quantity unidentified discrete} and \Ccode{action building/producing}. 
\Spair{Pairs} much more frequently mention the specific number of units/buildings being produced, such as \quotate{6}{These two forges come up} rather than an unknown number of units/buildings like \quotate{2}{An extra few gateways going down...} 
When discussing \Ccode{upgrades}, there are only 3 co-occurrences with \Ccode{unidentified discrete}, while there are 34 co-occurrences with \Ccode{identified discrete}.
This difference suggests that it is crucial for an explanation system to provide precise numbers when discussing upgrades.

%\boldify{Further evidence for the above claim can be found by comparing ID and UID, as they have similar occurrence for most categories except for action-building and production object}

Other examples of the co-occurrence of \Ccode{unspecified objects} and \Ccode{quantity comparative} were vague references to units, such as \quotate{3}{he already lost too many units and too long on his econ to make this strategy work anymore}

%\boldify{Unspecified and comparative have a high co-occurrence, and discussion of ``supply'' makes up the majority of this co-occurrence. May be related to constraints placed on the shoutcasters.}


%\boldify{Production and ID have very high occurrence (``how many things do i make?''. This means that there is a strong tendency to specify exactly how many workers or buildings the player possesses or should possess, while other objects are more likely to be counted imprecisely.}

\Ccode{Production objects} and \Ccode{quantity identified discrete} had a very high co-occurrence rate of 28\%.
176 instances of these co-occurrences were found in the corpus.
In some of these instances, \Spair{Pairs} give game state information about how many worker units players possess, such as \quotate{8}{21 probes against 13 drones}
Similarly, \Ccode{Pairs} also gave updates about resource counts, like \quotate{7}{Units lost tab actually tells the story, 12000 resources lost against the 8000 of Byun}
\Spair{Pairs} also used \Ccode{identified discrete} numbers to distinguish bases, like when \Spair{Pair 8} expressed that they \quotateUnattrib{don't understand why Showtime took his 4th base on the left side..}
\Ccode{Production objects} and \Ccode{quantity identified discrete} also co-occurred when describing combat, such as \Spair{Pair 1} stating jjakji was \quotateUnattrib{Going to force in a stalker warp and kill 8 probes..}
Given the high co-occurrence rate of \Ccode{production objects} and \Ccode{quantity identified discrete}, and the variety of instances that make up these co-occurrences, it is essential for the future explanation system to use \Ccode{identified discrete quantities} when discussing \Ccode{production objects}.

Alternatively, if \Spair{Pairs} were to mispredict, it could create confusion between expectation of action and interpretation of events (cognitive disequilibrium~\cite{lim2009assessing}) within their invisible audience, which might explain why there was such a low frequency of \LimDey{Why}.
Essentially, \Spair{Pairs} may only have been willing to make predictions when very confident, due to risk aversion.

\boldify{``Why'' would shoutcasters use a patch, in a general sense? 
Remember that CUES are agent actions, amidst the chaos of an environment, so they may require some support to find, but are worth the effort.
Therefore, navigations among patches and cues they were using suggests to us what THEY think is important. 
However, we did not interview, so our view is limited, but still useful.
}

First, let us briefly consider \emph{why} a shoutcaster would navigate to a different patch.
Remember that the \emph{prey} in our case is the agent's decision process, thus the \emph{cues} would be [evidence of] the agents' actions.
The navigations of the \Spair{Pairs} illuminated what \emph{THEY} thought was important within the information interface as they search for these cues.
We observed many cases where a \Spair{Pair} used a patch as a visual aid for discussion, but since the structure of our study did not allow us to interview them, we could not identify the reason with certainty.
However, we posited that some of the navigations allowed the \Spair{Pair} to learn something to inform commentary, while others \emph{clarified} or \emph{quantified} something for the viewer, which the \Spair{Pair} could have known before the navigation.

\boldify{GOAL: Some discussion about the planning depth associated with building.  Tom is interested to learn about how building differs from fighting in description, seeming to hypothesize that choosing to fight and how to fight is more of a one-shot decision problem, while building is more sequential.}
\FIXME{JED This sounds like we should look at co-occurring ordering with fighting and building and see what we see}

\boldify{GOAL: choosing the right level of abstraction. Shoutcasters have to use a sort of mental grammar that transforms clicks into a higher level of abstraction that they think explainees want to converse in. (clicks -> units moving -> reaver drop). This is important because the agent may do something, then justifies it by describing the 5000 clicks it performed, meanwhile the human does not care about that low level representation.}
\FIXME{JED yeah im still not sure how we stab at this. Maybe we discuss in the future work section?}

\boldify{PRELIMINARY: look at how utterances are situated in time somehow. Pay special attention to how spatial and temporal codes compare.}

\boldify{Difficulty with ambiguous language}
Spatiotemporal ``here''
Creep does many things
Knowledge is gained in many ways, some from the game state, from from PAST MATCHES
mirror matches

\boldify{Knowledgeable audience members may already know the answers to the questions ``Why'' and ``Why did not,'' explaining why shoutcasters would not need to answers these questions.}

Coding results showed that few shoutcaster explanations answered the questions ``Why'' and ``Why did not.''
It is expected that the audience of shoutcasted tournaments are knowledgeable fans, if they sought out and found these tournament videos.
If an experienced player has been given information about what happened in the game, they may be able to understand why players took certain actions.
Therefore, shoutcasters might not need to give explanations to the questions ``Why'' and ``Why didn't.''

\boldify{They seem to use popups mostly as a visual aid for the viewer.}
In our coding process, we considered something a ``Visual Aid,'' if the navigation was explicitly related to a discussion the casters were having.
When this occurs, it can be unclear if the ``Visual Aid'' is for the caster to uncover information about the game state for their own purpose, to reveal information to convince the viewer of something, or some combination of the two.
We observed 10 navigations to a popup, 7 of which were to the Units Lost popup, and the remaining 3 were to an income related overlay (1 was to the timeline graph described previously).
Of these 10 navigations, all but one, whose purpose was unknown, seemed to have the purpose of providing a visual aid.

\boldify{Some shoutcasters have diff patches available from other shoutcasters, and ALL of them have patches different from the people they're explaining to. So they paste some of their special-shoutcaster patch content onto the HUD visible to explainees to help explain stuff}
So far, we have focused our discussion on the HUD built-in to Starcraft 2.
As discussed previously, the HUDs shoutcasters use are augmented a bit from the basic observer interface we have discussed so far.
In our data we observed 6 different HUDs, and here we describe their similarities and differences.
%FIXME need to really nail down how many huds we saw and which have what properties and put a fine point on this paragraph. Also should mention that not all the casters had access to the same patches in the same way (e.g. 3/5 upgrade navigations come from the same video.  If the others had upgrade info available passively, that would explain why lopsided frequency. Also explains infrequent use of timeline charts (only available in one of the views)
%FIXME maybe typify the things that make it onto the HUD from the tab? are they all current state?
First, additional information from some of the tabs described above often makes it onto the HUD (e.g. the entire contents of the Income tab).
Additionally, some HUDs increase the visibility of events occurring on the minimap (e.g. when a structure is completed).
%Last, the HUD used by the casters who are working on the World Championship Series (WCS), shown in Figure~\ref{fig:WCS}, adds two additional visualizations: a graph of income vs time, and an in depth look at units lost. 

% Session 1  : WCS
% Session 2  : WCS
% Session 3  : AfreecaTV
% Session 4  : WESG
% Session 5  : jinair
% Session 6  : Kespa
% Session 7  : WESG
% Session 8  : gfuel
% Session 9  : WCS
% Session 10 : WESG

%IFT description from background (became replaced by introduction)
Constructs of IFT included the predator, the human, seeking their prey, the information.
The environment topology is made up of information patches.
Users navigated between the information patches by traversing links.
Cues in the information environment, such as words, are associated with the links.
Cues give information about what predators might obtain by traversing the links~\cite{fleming2013information}.
The user's underlying goal is to navigate in a way that maximizes value of knowledge received, while minimizing the cost of interaction.
Value can be estimated by using cues. However, estimated and actual value can be different~\cite{piorkowski2016foraging}.


**This parag is about aggregation.  MMB doesn't remember where it came from: was either RQ1 or RQ2:

The most common change from this was when items were being lost or in danger of being lost.
Then, some \Spair{pairs} appeared to swap to a visualization more suited for current state's \emph{environment}.
In both of these situations, \Spair{pairs} appeared to prefer visualizations with little aggregation.
The second most common change was to adopt a player's \emph{sensors} to understand the information gained or available at the time the player had made a key decision.
\emph{Performance} measures about past states were rarely consulted outside of settings where fighting had just ended.
Notably, many of these past state visualizations of performance measures used more data aggregation.

**These next 2 parags came from the Implications section of RQ3:

\boldify{More about satisficing, and how it may pertain to XAI}

There seems to be an inherent imbalance between askers and answerers, and it could be that askers \emph{know} this and will accept that some questions may be ignored or insufficiently addressed if they prove too challenging.
To illustrate, imagine a young child asking their parent ``Why...'' many times in a day; at some point the parent then responds ``Because that's how it is.''
In this example, the answer will probably be accepted despite not actually containing any reasoning.
The extent to which satisficing is acceptable for explanation systems remains to be seen, but it may prove necessary when time or resource costs do not permit providing the ``best available argument.''
\FIXME{JED This paragraph is still just D1 level, can probably also be shortened. Also, does the analogy read, and can it be improved?}

\boldify{Combine hypotheses:
H1: while our testers may not be in real-time like shoutcasters, messing with navigation links is clearly a significant disruption in workflow.
H2: COGNITIVE and RESOURCE costs are analogous, so really crystallizes how hard it is to 1. determine the correct ``linkage'' and 2. find the right pair of times to link
H3+4: Satisficing is common in this domain, and takes several forms}

While the \Spair{Pairs} faced a task that is perhaps more difficult than users of a future explanation system, Hypothesis 1 indicates that fetching an explanation from it may cause significant disruption in workflow for the tester.
Similarly, fetching an explanation may require high \emph{resource} cost, since cognitive costs are analogous and Hypothesis 2 indicates that those costs are high.
Unifying Hypotheses 3 and 4, we observe that ``satisficing'' appears to be prevalent in this domain, meaning that suboptimal options are deemed acceptable because they are available.
\FIXME{JED This paragraph is still just D1 level, can probably also be shortened.}


==> tables/TableWhyDidnt.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{@{}p{1\linewidth}@{}}
		\textit{\textbf{\LimDey{Why-didn't} answers}}                   
        \tabularnewline \hline
		In the midst of trying to defend this position properly, he has not put a new one down.
                \tabularnewline \hline
		The probe already left a while ago so we knew it wasn't going to be a pylon rush. 
                \tabularnewline \hline
The ling, he already lost too many units and too long on his econ to make this strategy work anymore.
                \tabularnewline \hline
Then again he hasnt scouted anything though, so this is more like a blind thing to make sure he's going to be able to deal with the banshees?
                \tabularnewline \hline
He's got the money for it, but he's focusing so hard on this production. 
                \tabularnewline \hline
I suppose you could argue that Innovation could have made a factory to the right side of the map or the base I should say but this is so standard it's hardly worth fighting.
	\end{tabular}
	\caption{All instances of answers to \LimDey{Why-didn't} questions, from Lim \& Dey coding.}
	\label{table:whyDidnt}   	
\end{table}

==> z-DraftCommands.tex <==
\usepackage{fancyhdr}
\pagestyle{fancy}
 
\fancyfoot{}
\renewcommand{\footrulewidth}{1pt}
\pagenumbering{arabic}
\lfoot{Page~\thepage}
\cfoot{\currenttime~GMT~(PST is GMT-07:00)}
\rfoot{\today}


\newcommand{\boldify}[1]{\textbf{**#1}}
\newcommand{\FIXME}[1]{\fbox{\parbox{\linewidth}{\textbf{FIXME} #1}}}

